Aguvis: Unified Pure Vision Agents for Autonomous GUI Interaction

Automating GUI tasks remains challenging due to reliance on textual representations, platform-specific action spaces, and limited reasoning capabilities. We introduce Aguvis, a unified vision-based framework for autonomous GUI agents that directly operates on screen images, standardizes cross-platform interactions and incorporates structured reasoning via inner monologue. To enable this, we construct Aguvis Data Collection, a large-scale dataset with multimodal grounding and reasoning annotations, and develop a two-stage training pipeline that separates GUI grounding from planning and reasoning. Experiments show that Aguvis achieves state-of-the-art performance across offline and real-world online benchmarks, marking the first fully autonomous vision-based GUI agent that operates without closed-source models. We open-source all datasets, models, and training recipes at https://aguvis-project.github.io to advance future research.

==> tables/ablation_ov_mobile_to_web.tex <==
\begin{table}[h!]
\centering
\caption{Ablation Study of AGUVIS-OV-G on MM-Mind2Web.}
\label{tab:aguvig_mm_mind2web}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccc}
\toprule
\multirow{2}{*}{\textbf{$\ourmodel_{\textsc{ov}}$}} & \multicolumn{3}{c}{\textbf{MM-Mind2Web}} \\
\cmidrule(lr){2-4}
                     & \textbf{Cross-Task} & \textbf{Cross-Website} & \textbf{Cross-Domain} \\
\midrule
Web + Mobile (Stage 2 Equivalent) & 55.3 & 50.0 & 50.8 \\
Web Only                          & 40.4 & 38.1 & 40.4 \\
Mind2Web Only                     & 43.4 & 39.0 & 40.7 \\
\bottomrule
\end{tabular}
}
\end{table}


==> tables/hyperparams.tex <==
\begin{table}[!t]
\centering
\small
    \begin{tabular}{l | c c}
    \toprule
    Hyperparameters & Grounding Training & Planning \& Reasoning training \\
    \midrule
    Batch Size & 128 & 128 \\
    Initial Learning Rate & 1e-5 & 1e-5 \\
    Learning Rate Decay & \multicolumn{2}{c}{Cosine Scheduler} \\
    Warmup Ratio & \multicolumn{2}{c}{0.1} \\
    \bottomrule
    \end{tabular}
    \caption{
    Hyperparameters.
    }
\label{tab:meter_params}
\end{table}

==> tables/llava_ov_m2w.tex <==
\begin{table}[htbp]
\centering
\caption{Performance comparison on Multimodal Mind2Web across different methods and evaluation settings.\zekun{check num.}}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccc|ccc|ccc}
\toprule
\bf Models & \multicolumn{3}{c|}{\textbf{Cross-Task}} & \multicolumn{3}{c|}{\textbf{Cross-Website}} & \multicolumn{3}{c}{\textbf{Cross-Domain}} \\
 &\textbf{Ele.Acc} & \textbf{Op.F1} & \textbf{Step SR} & \textbf{Ele.Acc} & \textbf{Op.F1} & \textbf{Step SR} & \textbf{Ele.Acc} & \textbf{Op.F1} & \textbf{Step SR} \\
\midrule
LLaVA-OV-7B-P (Ours) & 60.5 & 88.0 & 55.3& 57.7 & 86.8 & 50.0 & 55.9 & 86.9 & 50.82 \\
\bottomrule
\end{tabular}
}
\end{table}

==> tables/llava_ov_results.tex <==
\begin{table}[htbp]
    \centering
        \small
        \captionof{table}{Performance of \ourmodel based on LLaVA-OneVision backbone. We report the average score on ScreenSpot and the step success rate of each split in Multimoda-Mind2Web. These results demonstrate that our framework and data recipe are model independent and the planning stage can largely improve the performance of both grounding and planning ability.}
        % \resizebox{\textwidth}{!}{%
        \begin{tabular}{lcccc}
            \toprule
            \multirow{2}{*}{\bf Models} & \bf ScreenSpot & \multicolumn{3}{c}{\bf MM-Mind2Web} \\ 
            & Average & Task & Website & Domain \\
            \midrule
            Previous SOTA & 73.3 & 39.4 & 36.5 & 42.0 \\
            $\ourmodel_{\textsc{ov}}$-G-7B & 70.0 & 43.4 & 39.0 & 40.7 \\
            $\ourmodel_{\textsc{ov}}$-7B & 81.2 & 55.3 & 50.0 & 50.8\\
            \bottomrule
        \end{tabular}
        % }
    \label{tab:llava_ov}
\end{table}


==> tables/llava_ov_screenspot_results.tex <==
\begin{table}[ht]
    \caption{LLaVA-ov results.\zekun{Need a new name of LLaVA?}}
    \centering
     \resizebox{\textwidth}{!}{%
    \begin{tabular}{lccccccccc}
        \toprule
        \multirow{2}{*}{\bf Models} & \multicolumn{2}{c}{\textbf{Mobile}} & \multicolumn{2}{c}{\textbf{Desktop}} & \multicolumn{2}{c}{\textbf{Web}} & \multirow{2}{*}{\textbf{Average}} \\
        & \textbf{Text} & \textbf{Icon/Widget} & \textbf{Text} & \textbf{Icon/Widget} & \textbf{Text} & \textbf{Icon/Widget} & \\
        \midrule
        % \multirow{5}{*}{-} 
        % UGround & 82.8 & 60.3 & 82.5 & 63.6 & 80.4 & 70.4 & 73.3 \\
        LLaVA-OV-7B-G (ours) & 70.0 & 59.4 & 89.7 & 65.0 & 72.2 & 64.1 & 70.0 \\
        LLaVA-OV-7B-P (ours) & 89.4 & 78.6 & 89.7 & 67.9 & 85.7 & 69.4 & 81.2 \\
        \bottomrule
    \end{tabular}
    }
    \label{tab:llava_ov}
\end{table}

